Integrating Deep Learning in Domain Sciences at Exascale

This paper presents some of the current challenges in designing deep learning artificial intelligence (AI) and integrating it with traditional high-performance computing (HPC) simulations. We evaluate existing packages for their ability to run deep learning models and applications on large-scale HPC systems efficiently, identify challenges, and propose new asynchronous parallelization and optimization techniques for current large-scale heterogeneous systems and upcoming exascale systems. These developments, along with existing HPC AI software capabilities, have been integrated into MagmaDNN, an open-source HPC deep learning framework. Many deep learning frameworks are targeted at data scientists and fall short in providing quality integration into existing HPC workflows. This paper discusses the necessities of an HPC deep learning framework and how those needs can be provided (e.g., as in MagmaDNN) through a deep integration with existing HPC libraries, such as MAGMA and its modular memory management, MPI, CuBLAS, CuDNN, MKL, and HIP. Advancements are also illustrated through the use of algorithmic enhancements in reduced- and mixed-precision, as well as asynchronous optimization methods. Finally, we present illustrations and potential solutions for enhancing traditional compute- and data-intensive applications at ORNL and UTK with AI. The approaches and future challenges are illustrated in materials science, imaging, and climate applications.

==> reduced_precision.tex <==
\subsection{Reduced Precision}
Training deep neural networks commonly does not require high precision arithmetic where FP32 or lower precision can significant improve performance to reducing time for training without sacrificing accuracy.
%
There are several formats for reduced precision. One is 16-bit FP16 with 11 bits of accuracy but limited dynamic range, another is 16-bit Bfloat16 with 8 bits of accuracy but same dynamic range as FP32, and TF32  that has same dynamic range as FP32 but with 11 bits of accuracy.
%
Special hardware accelerators can take advantage of reduced or mixed precision arithmetic. For example, the Tensor Core on  NVIDIA Volta GPU accelerates $4 \times 4$ 
matrix multiplication $D_{32} = C_{32} + A_{16} * B_{16}$, where
$A_{16}$ and $B_{16}$ are $4 \times 4$ matrices are in FP16 with 11 bits of accuracy.
%
The peak performance on Volta GPU is 125 TFLOPS, which is 8 times the peak performance
for FP32.
%
There is much interest in exploiting reduced precision arithmetic on the Tensor Core.
%
Using LU factorization performed in reduced precision as a preconditioner of Krylov iterative method can
accelerate the solution of a large dense linear system of equations~\cite{Azzam_FP16}. 
Tensor Core can also be used in performing FFT~\cite{Kwai_FFT}.
%
Note that a matrix in FP32 can be well approximated as the scaled sum of two FP16 matrices
\begin{equation}
A_{32} \approx a1_{32} * A1_{16} + a2_{32} * A2_{16}
\label{eqn:fp32_fp16}
\end{equation}
where $a1_{32}$, $a2_{32}$ are in FP32.
The scaling by $a1_{32} (a2_{32})$ ensures $A1_{16}  (A2_{16})$ is within the
limited dynamic range of FP16. 
%
Conceptually, $A1_{16}$ roughly captures the 3 most significant decimal digits, and $A2_{16}$ the
next 3 lower significant decimal digits.
%
If $A_{32}$ is already well-scale, then one can expect $a1_{32} = 1$ and $a2_{32}=2^{-11} * a1_{32}$.
Matrix multiplication of two FP32 matrices can be approximated by 3 matrix multiplications of
FP16 matrices on Tensor Core (Appendix A), which may give a theoretical speedup of 8/3 times on Volta GPU.
%
For another perspective, the  equation (\ref{eqn:fp32_fp16}) suggests the form of operations in deep
neural network are theoretically able to well approximate operations of FP32 using careful use of mixed precision operations in FP16.

